3D Point Cloud Denoising via Bipartite Graph Approximation and Reweighted Graph Laplacian

Point cloud is a collection of 3D coordinates that are discrete geometric samples of an object's 2D surfaces. Imperfection in the acquisition process means that point clouds are often corrupted with noise. Building on recent advances in graph signal processing, we design local algorithms for 3D point cloud denoising. Specifically, we design a reweighted graph Laplacian regularizer (RGLR) for surface normals and demonstrate its merits in rotation invariance, promotion of piecewise smoothness, and ease of optimization. Using RGLR as a signal prior, we formulate an optimization problem with a general lp-norm fidelity term that can explicitly model two types of independent noise: small but non-sparse noise (using l2 fidelity term) and large but sparser noise (using l1 fidelity term). To establish a linear relationship between normals and 3D point coordinates, we first perform bipartite graph approximation to divide the point cloud into two disjoint node sets (red and blue). We then optimize the red and blue nodes' coordinates alternately. For l2-norm fidelity term, we iteratively solve an unconstrained quadratic programming (QP) problem, efficiently computed using conjugate gradient with a bounded condition number to ensure numerical stability. For l1-norm fidelity term, we iteratively minimize an l1-l2 cost function sing accelerated proximal gradient (APG), where a good step size is chosen via Lipschitz continuity analysis. Finally, we propose simple mean and median filters for flat patches of a given point cloud to estimate the noise variance given the noise type, which in turn is used to compute a weight parameter trading off the fidelity term and signal prior in the problem formulation. Extensive experiments show state-of-the-art denoising performance among local methods using our proposed algorithms.

==> denoising.tex <==

Given two neighboring nodes $i,j\in\mathcal{E}$ for a constructed point cloud graph $\mathcal{G}=(\mathcal{V,E})$, when the underlying 2D surface is smooth, the corresponding (consistently oriented) surface normals at nodes $i$ and $j$ should be similar. 
Hence the piecewise smoothness (PWS) of the point cloud surface can be measured using GTV of surface normals over $\mathcal{G}$ as follows:
\begin{equation}
|\vert\mathbf{n}|\vert_{\text{GTV}}=\sum_{i,j\in\mathcal{E}}w_{i,j}|\vert\mathbf{n}_{i}-\mathbf{n}_{j}|\vert_1,
\label{eq:main_TV}
\end{equation}
where $\mathbf{n}_{i}\in \mathbb{R}^{3}$ is the surface normal at node $i$. Now we can formulate our point cloud denoising problem as a minimization of the defined GTV while keeping the points close to their original locations. 
\red{this is defined earlier in preliminaries, right?}
Denote the 3D coordinate of a point/node $i$ by a column vector $\mathbf{p}_{i}$ and $\mathbf{p}~=~\begin{bmatrix} \mathbf{p}_{1}^{T} & \hdots & \mathbf{p}_{|\mathcal{V}|}^{T} \end{bmatrix}^T$, where $|\mathcal{V}|$ is the number of points in the point cloud. Here, $\mathbf{p}$ is the optimization variable, and $\mathbf{n}_{i}$'s are functions of $\mathbf{p}$. 
Unfortunately, using state-of-art surface normal estimation methods, each $\mathbf{n}_{i}$ is a nonlinear function of $\mathbf{p}_{i}$ and its neighbors. 
Hence, it is difficult to formulate a simple convex optimization problem using GTV in (\ref{eq:main_TV}).

To overcome this difficulty, we first partition the set of 3D points into two classes (say red and blue). 
To compute surface normal of a red point, we use only coordinates of the red point and its neighboring blue points, resulting in a linear relationship between surface normals and 3D coordinates of red points. 
Towards this goal, we compute a bipartite graph approximation of the original graph $\mathcal{G}$ as follows. 


\subsection{Bipartite Graph Approximation}

A bipartite graph $\mathcal{B}=(\mathcal{V}_1,\mathcal{V}_2,\mathcal{E}')$ is a graph whose nodes are divided into two disjoint sets $\mathcal{V}_1$ and $\mathcal{V}_2$ (\textit{e.g.}, red and blue nodes respectively), such that each edge connects a node in $\mathcal{V}_1$ to one in $\mathcal{V}_2$. 
Given an original graph $\mathcal{G}~=~(\mathcal{V},\mathcal{E})$, our goal is to find a bipartite graph $\mathcal{B}$ that is ``closest" to $\mathcal{G}$ under a chosen metric.

First, we assume that the generative model for graph-signals $\mathbf{f}$ on a given graph $\mathcal{G}$ is a \textit{Gaussian Markov random field} (GMRF) \cite{rue2005}. 
Specifically, $\mathbf{f}\sim\mathcal{N}(\mathbf{\mu},\mathbf{\Sigma})$, where $\mathbf{\mu}$ is the mean vector, and $\mathbf{\Sigma}$ is the covariance matrix specified by the graph Laplacian matrix $\mathbf{L}$ of $\mathcal{G}$, \textit{i.e.}, $\Sigma^{-1}~=~\mathbf{L}+\delta\mathbf{I}$, where $1/\delta$ is interpreted as the variance of the DC component for $\mathbf{f}$. 
For simplicity, we assume $\mathbf{\mu}=\mathbf{0}$.

We now find a graph $\mathcal{B}$ whose probability distribution $\mathcal{N}_B(\mathbf{0},\mathbf{\Sigma}_{\mathcal{B}})$ under the same GMRF model is closest to $\mathcal{N}(\mathbf{0},\mathbf{\Sigma})$ in terms of  \textit{Kullback-Leibler Divergence} (KLD) \cite{duchi2007}:
\begin{equation}
D_{KL}(\mathcal{N}||\mathcal{N}_{\mathcal{B}})=\frac{1}{2}(\text{tr}(\mathbf{\Sigma}_{\mathcal{B}}^{-1}\mathbf{\Sigma})+\text{ln}|\mathbf{\Sigma}_{\mathcal{B}}\mathbf{\Sigma}^{-1}|-|\mathcal{V}|),
\label{eq:KLD}
\end{equation}
where $\Sigma_{\mathcal{B}}^{-1}~=~\mathbf{L}_{\mathcal{B}}+\delta\mathbf{I}$ is the precision matrix of the GMRF specified by $\mathcal{B}$, and $\mathbf{L}_{\mathcal{B}}$ is the graph Laplacian matrix of $\mathcal{B}$. To minimize (\ref{eq:KLD}), we use an iterative greedy algorithm similar to the one proposed in \cite{zeng2017} as follows.

Given a non-bipartite graph $\mathcal{G}$, we build a bipartite graph $\mathcal{B}$ by iteratively adding one node at a time to one of two disjoint sets ($\mathcal{V}_{1}$ and $\mathcal{V}_{2}$) and removing the edges within each set. 
First, we initialize one node set $\mathcal{V}_1$ with one randomly chosen node, and $\mathcal{V}_{2}$ is empty. 
Then, we use \textit{breadth-first search} (BFS) \cite{ba3na2002} to explore nodes within one hop in $\mathcal{G}$. 
To determine to which set between $\mathcal{V}_1$ and $\mathcal{V}_2$ the next node should be assigned, we calculate KLD $D_{KL}^{i}$ where $i=1,2$, assuming the node is assigned to $\mathcal{V}_1$ or $\mathcal{V}_2$ respectively. 
The node is assigned to $\mathcal{V}_{1}$ if $D_{KL}^{2}>D_{KL}^{1}$, and to $\mathcal{V}_2$ otherwise. 
If $D_{KL}^{2}=D_{KL}^{1}$, then the node is alternately allocated to $\mathcal{V}_1$ and $\mathcal{V}_2$, so that the resulting sizes of the two node sets will be balanced.

An example for the bipartite graph approximation is shown in Fig.\;\ref{fig:bipartite_graph}. 
Here, we construct the original $k$-NN graph ($k=6$) using a small portion of Bunny point cloud model in~\cite{levoy2005}.

\begin{figure}[t]
\centering
\subfloat[original graph]{
\includegraphics[width=0.23\textwidth]{original}
\label{fig:pcd-day}}
%\hspace{-6pt}
\subfloat[bipartite graph]{
\includegraphics[width=0.23\textwidth]{bipar}
\label{fig:pcd-on}}
%\hspace{-6pt}
\caption[]{An example for bipartite graph approximation.} %~\cite{bernardini1999}
\label{fig:bipartite_graph}
%\vspace{-10pt}
\end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[width=1.1in]{normal_vect} %width=1.65in,
 \vspace{-10pt}
 \caption{Illustration of the normal vector estimation at a red node.}
 \label{fig:normalvec}
\vspace{-15pt}						
  \end{figure} 
  
\subsection{Normal Vector Estimation}
\label{sec:normalvector}

We describe how we define $\mathbf{n}_{i}$ for a red node $i$. 
\red{u now have a constructed bipartite graph, so for each red node $i$, it should \textit{only} have connected neighbors in blue. r u assuming each red node has \textit{at least} two blue neighbors (connected in the bipartite graph), and u choose two?}
We identify two nearest connected blue node neighbors (named $k$ and $l$) that are not on a straight line with red node $i$ to compute a perpendicular vector to a 2D plane defined by nodes $i$, $k$ and $l$ (see Fig.\;\ref{fig:normalvec} for an illustration). 
The corresponding 3D coordinates of nodes $i$, $k$, and $l$ are denoted by $\mathbf{p}_i=\begin{bmatrix} x_i & y_i & z_i \end{bmatrix}^T$,  $\mathbf{p}_k=\begin{bmatrix} x_k & y_k & z_k \end{bmatrix}^T$, and $\mathbf{p}_l=\begin{bmatrix} x_l & y_l & z_l \end{bmatrix}^T$ respectively. 
We define the normalized perpendicular vector $\mathbf{n}_i$ to that plane as the surface normal at node $i$, computed as:
\begin{equation}
\mathbf{n}_i=\frac{[\mathbf{p}_i-\mathbf{p}_k]\times [\mathbf{p}_k-\mathbf{p}_l]}{|\vert[\mathbf{p}_i-\mathbf{p}_k]\times [\mathbf{p}_k-\mathbf{p}_l]|\vert_2},
\label{eq:cross_prod}
\end{equation}
where `$\times$' represents the vector cross product operator. 
We rewrite the cross product in (\ref{eq:cross_prod}) as follows:
 
\begin{equation}
\begin{split}
[\mathbf{p}_i-\mathbf{p}_k]\times [\mathbf{p}_k-\mathbf{p}_l]=\underbrace{\begin{bmatrix}0 & z_k-z_l & y_l-y_k \\
                         z_l-z_k & 0 &x_k-x_l \\
                         y_k-y_l & x_l-x_k & 0\end{bmatrix}}_{\mathbf{C}_i}\begin{bmatrix}x_i\\y_i\\z_i \end{bmatrix}\\+
                         \underbrace{\begin{bmatrix}-y_k(z_k-z_l)-z_k(y_l-y_k)\\-x_k(z_k-z_l)-z_k(x_k-x_l)\\-x_k(y_k-y_l)-y_k(x_l-x_k)\end{bmatrix}}_{\mathbf{d}_i}\\
 \end{split}
 \label{eq:linear}
 \end{equation}
Thus, normal vector $\mathbf{n}_{i}$ can be re-written as:
 \begin{equation}
 \mathbf{n}_i=\frac{\mathbf{C}_{i}\mathbf{p}_{i}+\mathbf{d}_{i}}{|\vert\mathbf{C}_{i}\mathbf{p}_{i}+\mathbf{d}_{i}|\vert_2}.
 \label{eq:norm_vec}
 \end{equation}
 
The orientations of the normal vectors for a local neighborhood of red nodes computed using (\ref{eq:norm_vec}) are not necessarily consistent. 
To achieve consistent orientations of the surface normals, we fix the orientation of one normal vector and propagate this information to neighboring red points. 
Specifically, we use \textit{minimum spanning tree} (MST) \cite{hoppe1992} for propagation. 
First, a $k$-NN graph of red nodes is constructed with $w_{i,j}~=~1-|\mathbf{n}_{i}^{T}\mathbf{n}_{j}|$, where $\mathbf{n}_{i}$ and $\mathbf{n}_{j}$ are computed using~(\ref{eq:norm_vec}).
Then, an arbitrary node of the graph is assumed to be the tree root, and the normal is propagated to its children nodes recursively. When the normal direction is propagated from node $i$ to node $j$, if $\mathbf{n}_{i}^{T}\mathbf{n}_{j}$ is negative, then the direction of $\mathbf{n}_{j}$ is reversed; otherwise it is left unchanged. 

Consistently oriented normal vectors can now be written as:
 \begin{equation}
 \mathbf{n}_i=\left(\frac{\mathbf{C}_{i}\mathbf{p}_{i}+\mathbf{d}_{i}}{|\vert\mathbf{C}_{i}\mathbf{p}_{i}+\mathbf{d}_{i}|\vert_2}\right)\alpha,
 \label{eq:norm_vec_ori}
 \end{equation}
where $\alpha$ is 1 or $-1$ according to the consistent normal orientation.

In this paper, for simplicity we assume that the scalar values $\alpha$ and $|\vert\mathbf{C}_{i}\mathbf{p}_{i}+\mathbf{d}_{i}|\vert_2$ remain constant when $\mathbf{p}_{i}$ is being optimized. 
Hence, surface normal $\mathbf{n}_i$ can be written as a linear function of 3D coordinates $\mathbf{p}_i$ of the point $i$. 
Specifically,
\begin{equation}
\mathbf{n}_{i}=\mathbf{A}_{i}\mathbf{p}_{i}+\mathbf{b}_{i},
\label{eq:normal_linear}
\end{equation}
where $\mathbf{A}_{i}~=~\mathbf{C}_{i}\alpha^{in}/|\vert\mathbf{C}_{i}\mathbf{p}_{i}^{in}+\mathbf{d}_{i}|\vert_2$ and $\mathbf{b}_{i}~=~\mathbf{d}_{i}\alpha^{in}/|\vert\mathbf{C}_{i}\mathbf{p}_{i}^{in}+\mathbf{d}_{i}|\vert_2$. Here $\mathbf{p}_{i}^{in}$ is the initial vector of $\mathbf{p}_{i}$ and $\alpha^{in}$ is the value of $\alpha$ computed at $\mathbf{p}_{i}=\mathbf{p}_{i}^{in}$.

%\begin{figure}[t]
%\centering
%\subfloat[]{
%\includegraphics[width=0.235\textwidth]{without_ori}
%\label{fig:pcd-day}}
%\hspace{-10pt}
%\subfloat[]{
%\includegraphics[width=0.235\textwidth]{with_ori}
%\label{fig:pcd-on}}
%\hspace{-10pt}
%\caption[]{surface normals a) before b) after consistent %orienting alignment.} %~\cite{bernardini1999}
%\label{fig:normal_ori}
%\vspace{-15pt}
%\end{figure}

\subsection{Optimization Framework}
\label{sec:optimization}

After computing surface normals for each red node, we construct a \textit{new} $k$-NN graph $\mathcal{G}=(\mathcal{V}_{1},\mathcal{E}_{1})$ for red nodes, where $\mathcal{V}_{1}$ is the set of red nodes and $\mathbf{\mathcal{E}_{1}}$ is the set of edges connecting neighboring red nodes. 
Given $\mathcal{G}$, we define a $l_2$-$l_1$-norm minimization problem for denoising:

\begin{equation}
\min_{\mathbf{p},\mathbf{n}}|\vert\mathbf{q-p}\vert|_{2}^{2} + \gamma\sum_{i,j \in \mathcal{E}_1} w_{i,j} \| \mathbf{n}_{i} - \mathbf{n}_{j} \|_1 
\label{eq:main_opt}
\end{equation}
subject to linear constraint (\ref{eq:normal_linear}), where $\gamma$ is a weight parameter that trades off the fidelity term and GTV prior, and $w_{i,j}$ is the edge weight between nodes $i$ and node $j$ as defined in (\ref{eq:edge_weight}). 

To solve (\ref{eq:main_opt}), we first introduce new variables $\mathbf{m}_{i,j}$:
\begin{equation}
\begin{split}
&\quad \min_{\mathbf{p,m}}|\vert\mathbf{q-p}\vert|_{2}^{2} + \gamma \sum_{i,j \in \mathcal{E}_1} w_{i,j} \| \mathbf{m}_{i,j} \|_1 \\
&\quad \text{s.t.} \hspace{10pt} \mathbf{m}_{i,j} = \mathbf{n}_{i} - \mathbf{n}_{j}, 
\end{split}
\label{eq:main_opt_admm}
\end{equation}
again subject to constraint (\ref{eq:normal_linear}).
We next design an algorithm based on \textit{Alternating Direct Method of Multipliers} (ADMM) \cite{boyd2011} with a nested proximal gradient descent\cite{parikh2014} to solve (\ref{eq:main_opt_admm}).
We first write the linear constraint for each $\mathbf{m}_{i,j}$ in matrix form using our definition of $\mathbf{n}_{i}=\mathbf{A}_{i}\mathbf{p}_{i}+\mathbf{b}_{i}$ in~(\ref{eq:normal_linear}):
\begin{equation}
\begin{split}
\mathbf{m}&\quad =\mathbf{Bp+v},
\end{split}
\end{equation}
where $\mathbf{m}\in \mathbb{R}^{3|\mathcal{E}_1|}$, $\mathbf{B}\in \{\mathbf{A}_{i},\mathbf{0},-\mathbf{A}_{j}\}^{3|\mathcal{E}_1|\times3|\mathcal{V}_1|}$, $\mathbf{v}\in\{\mathbf{b}_{i}-\mathbf{b}_{j}\}^{3|\mathcal{E}_1|}$. Specifically, for each $\mathbf{m}_{i,j}$, the corresponding block row in $\mathbf{B}$ has all zero matrices except block entries $i$ and $j$ have $\mathbf{A}_{i}$ and $-\mathbf{A}_{j}$ respectively. Moreover, for each $\mathbf{m}_{i,j}$, the corresponding block entry in $\mathbf{v}$ is $\mathbf{b}_{i}-\mathbf{b}_{j}$. 
We can now rewrite (\ref{eq:main_opt_admm}) in ADMM scaled form as follows:
\begin{equation}
\begin{split}
\min_{\mathbf{p,m}}|\vert\mathbf{q-p}\vert|_{2}^{2}~+~\gamma\sum_{i,j\in \mathcal{E}_1} w_{i,j} \| \mathbf{m}_{i,j} \|_1 ~+\\
\frac{\rho}{2}|\vert\mathbf{Bp+v-m+u} |\vert_{2}^{2}+\text{const},
\end{split}
\label{eq:admm}
\end{equation}
where $\rho>0$ is a Lagrange multiplier. 
As typically done in ADMM, we solve (\ref{eq:admm}) by alternately minimizing $\mathbf{p}$ and $\mathbf{m}$ and updating dual variable $\mathbf{u}$ one at a time in turn until convergence.

\subsubsection{$\mathbf{p}$ minimization}

To minimize $\mathbf{p}$ having $\mathbf{m}^{k}$ and $\mathbf{u}^{k}$ fixed, we take derivatives of (\ref{eq:admm}) with respect to $\mathbf{p}$, set it to $0$ and solve for the closed form solution $\mathbf{p}^{k+1}$:
\begin{equation}
(2\mathbf{I}+\rho\mathbf{B}^{T}\mathbf{B})\mathbf{p}^{k+1}=2\mathbf{q}+\rho\mathbf{B}^{T}(\mathbf{m}^{k}-\mathbf{u}^{k}-\mathbf{v}),
\label{eq:p_mini}
\end{equation}
where $\mathbf{I}$ is an identity matrix. We see that matrix $2\mathbf{I}+\rho\mathbf{B}^{T}\mathbf{B}$ is positive definite (PD) for $\rho > 0$ and hence invertible. 
Further, the matrix is sparse and symmetric, hence (\ref{eq:p_mini}) can be solved efficiently via \textit{conjugate gradient} (CG) without full matrix inversion \cite{shewchuk1994}. 

\subsubsection{$\mathbf{m}$ minimization}

Keeping $\mathbf{p}^{k+1}$ and $\mathbf{u}^{k}$ fixed, the minimization of $\mathbf{m}$ becomes:
\begin{equation}
\min_{\mathbf{m}}\underbrace{\frac{\rho}{2}|\vert\mathbf{Bp}^{k+1}+\mathbf{v-m}+\mathbf{u}^{k} |\vert_{2}^{2}}_{f(\mathbf{m})}+\gamma\sum_{i,j\in \mathcal{E}_1} w_{i,j} \| \mathbf{m}_{i,j} \|_1,
\label{eq:m_mini}
\end{equation}
where the first term $f(\mathbf{m})$ is convex and differentiable, and the second term is convex but non-differentiable. We can thus use \textit{accelerated proximal gradient}~\cite{parikh2014} to solve (\ref{eq:m_mini}). The $f(\mathbf{m})$ has gradient $\Delta f$:
\begin{equation}
\Delta f(\mathbf{m})=-\rho(\mathbf{Bp}^{k+1}+\mathbf{v-m}+\mathbf{u}^{k}).
\label{eq: f_grad}
\end{equation}

We can now define a \textit{proximal mapping} $\text{prox}_{g,t}(\mathbf{m})$ for a convex, non-differentiable function $g()$ with step size $t$ as:
\begin{equation}
\text{prox}_{g,t}(\mathbf{m})=\text{arg}\min_{\theta}\left\{g(\theta)+\frac{1}{t}|\vert\theta-\mathbf{m}\vert|_{2}^{2}\right\}
\end{equation}
We know that for our weighted $l_{1}$-norm in (\ref{eq:m_mini}), the proximal mapping is just a soft thresholding function~\cite{parikh2014}:
\begin{equation}
\text{prox}_{g,t}(m_{i,j,r})=\begin{cases}
m_{i,j,r}-t\gamma w_{i,j} &\text{if} \hspace{5pt} m_{i,j,r}>t\gamma w_{i,j}\\
0 &\text{if} \hspace{5pt} \vert m_{i,j,r}\vert\leq t\gamma w_{i,j}\\
m_{i,j,r}+t\gamma w_{i,j} &\text{if} \hspace{5pt} m_{i,j,r}<t\gamma w_{i,j},
\end{cases}
\end{equation}
where $m_{i,j,r}$ is the $r$-th entry of $\mathbf{m}_{i,j}$. To adopt an accelerated proximal gradient approach, we then define (with initial point $\mathbf{m}^{(-1)}~=~\mathbf{m}^0$)
\begin{equation}
\mathbf{z}^k=\mathbf{m}^k+\frac{k-1}{k+2}\left(\mathbf{m}^k-\mathbf{m}^{k-1}\right),
\end{equation}
where $\mathbf{z}^k$ is an extrapolated point computed from the two previous solutions $\mathbf{m}^k$ and $\mathbf{m}^{k-1}$. We now update $\mathbf{m}^{k+1}$ using $\mathbf{z}^k$ as follows:
\begin{equation}
\mathbf{m}^{k+1}=\text{prox}_{g,t}(\mathbf{z}^{k}-t\Delta f(\mathbf{v}^{k})).
\label{eq:m_update}
\end{equation}
We compute (\ref{eq:m_update}) iteratively until convergence. \blue{An appropriate step size $t$ for a faster convergence can be selected based of the Libschitz continuity~\cite{combettes2005} of $\Delta f$ as follows.} 

\blue{We say that $\Delta f$ is Libschitz continuous if there is a real positive constant $K$ such that, for all real $\mathbf{m}_1, \mathbf{m}_2 \in \mathbb{R}^{3|\mathcal{E}_1|}$},
\begin{equation}
\blue{\norm{\Delta f(\mathbf{m}_1)-\Delta f(\mathbf{m}_1)}_2\leq K\norm{\mathbf{m}_1-\mathbf{m}_2}_2.}
\label{eq: Lip_conti}
\end{equation}
\blue{The smallest possible $K$ that satisfies (\ref{eq: Lip_conti}) is called Libschitiz constant $L$. Moreover, according to (\ref{eq: f_grad}), we can write}
\begin{equation}
\blue{\norm{\Delta f(\mathbf{m}_1)-\Delta f(\mathbf{m}_1)}_2=\rho\norm{\mathbf{m}_1-\mathbf{m}_2}_2}
\end{equation}
\blue{for all real $\mathbf{m}_1, \mathbf{m}_2 \in \mathbb{R}^{3|\mathcal{E}_1|}$, and therefore $\Delta f$ is Lipschitz continuous with $L=\rho$. As discussed in~\cite{parikh2014}, the accelerated proximal gradient algorithm has convergence rate $\mathcal{O}(1/k^2)$ when a step size $t\in (0,1/L]$ is used. This is theoretically the fastest possible convergence rate for first-order methods.} 
\subsubsection{$\mathbf{u}$-update}
Finally, we can update $\mathbf{u}^{k+1}$ simply:
\begin{equation}
\mathbf{u}^{k+1}=\mathbf{u}^{k}+(\mathbf{Bp}^{k+1}+\mathbf{v}-\mathbf{m}^{k+1}).
\label{eq:u_update}
\end{equation}
$\mathbf{p}$, $\mathbf{m}$ and $\mathbf{u}$ are iteratively optimized in turn using (\ref{eq:p_mini}), (\ref{eq:m_update}) and (\ref{eq:u_update}) until convergence.

Following the procedure in Section \ref{sec:normalvector} and \ref{sec:optimization}, two sets of nodes (\textit{i.e.}, red and blue) are alternately optimized until convergence.

==> inpainting.tex <==
The proposed hole filling framework consists of five main steps -- priority calculation (Section~\ref{sec:priority}), rigid template matching (Section~\ref{sec:rigid_matching}), denoising, non-rigid template matching and point transfer (Section~\ref{sec:transfer}) -- applied iteratively until the hole is filled. At each iteration, the highest-priority cube $\psi_{\mathbf{p}}$ centered on the fill front ($\mathbf{p} \in \delta \Omega$) is selected. The available points in this cube ($\psi_{\mathbf{p}} \cap \Phi$) are used as a template to search the source region $\Omega$. Then the denoising of the best-matching cube from the source region is performed. Afterword, a non-rigid transformation is applied to the denoised cube so that it further aligns with the template. Finally, this cube from the source region is used to transfer points to the hole, the fill front is updated, and the next iteration starts. The detail explanations of each step is in the remainder of this section. 
\begin{figure}[t]
                \centering
                \includegraphics[width=2.7in]{Normal_Vectors6}
               \caption{Illustration of several normal vectors in a typical $\psi_{\mathbf{p}}$.}
\label{fig:normal_vectors}					
\end{figure}
\subsection{Priority calculation}
\label{sec:priority}
Like the inpainting method in~\cite{Criminisi2004}, the proposed algorithm uses a best-first fill strategy that depends on the priority values assigned to each $\psi_{\mathbf{p}}$ for $\mathbf{p}\in \delta\Omega$. The assigned priority is biased towards those $\psi_{\mathbf{p}}$'s that seem to be on the continuation of ridges, valleys, and other surface elements that could more reliably be extended into the hole. 
For a given $\psi_{\mathbf{p}}$ for $\mathbf{p} \in \delta\Omega$, the priority $P(\mathbf{p})$ is defined as a product of two terms:
%\vspace{-5pt}
\begin{equation}
 P(\mathbf{p})=D(\mathbf{p})C(\mathbf{p}),
\label{eq:priority}
%\vspace{-5pt}
\end{equation}

where $D(\mathbf{p})$ is the data term and $C(\mathbf{p})$ is the confidence term. As in~\cite{Criminisi2004}, the confidence term $C(\mathbf{p})$ is defined as the number of available points in $\psi_{\mathbf{p}}$ ($C(\mathbf{p})=|\psi_{\mathbf{p}} \cap \Phi|$), in order to give higher priority to cubes with larger number of available points because they lead to more reliable template matching. 

The data term $D(\mathbf{p})$ depends on the structure of the data in $\psi_{\mathbf{p}}$. One of the main contributions of~\cite{Criminisi2004} was to realize that in the case of image inpainting, certain structures such as strong edges incident on the fill front may be more reliably extended into the hole compared to flat, textureless regions. Our goal here is to develop an analogous strategy for 3D point clouds. The challenge is that the image processing concepts such as contour normal and isophote, which allow for computation of the data term $D(\mathbf{p})$ in~\cite{Criminisi2004}, do not exist in the context of 3D point clouds. 

To overcome this challenge, we propose several new concepts. First we note that a ridge or a valley on a 3D surface may be considered as analogous to an edge in an image -- it is characterized by large variation in one direction (perpendicular to the edge/ridge/valley) and small variation in the other direction (parallel to the edge/ridge/valley). We measure variations in the point cloud $\psi_{\mathbf{p}}$ by examining \emph{surface normals}. \blue{For each point in $\psi_{\mathbf{p}}$, six nearest neighbors are used to fit a plane~\cite{hoppe1992}, and the unit normal vector to that plane is considered the surface normal vector at the corresponding point.}
An illustration is given in Fig.~\ref{fig:normal_vectors}, where the point cloud is represented as a surface for better visualization, and several normal vectors are indicated. 
%Plane fitting requires finding six nearest neighbors to each point in $\psi_{\mathbf{p}}$. The complexity of finding $k$-nearest neighbors in a point cloud is $\mathcal{O}(n + k\log{}n)$, where $n$ is the number of points in the point cloud, while finding the normal vector is an $\mathcal{O}(n)$ procedure~\cite{hoppe1992}. Normal vectors could also be obtained by first fitting a mesh to the point cloud and then computing the normals to the mesh faces. However, this would be more expensive since triangular mesh construction is an $\mathcal{O}(n^{2})$ procedure~\cite{zou2013}.

To identify a possible ridge/valley that is incident on the fill front, we measure the variation of normal vectors along the fill front. Specifically, for a given $\psi_{\mathbf{p}}$, the \emph{boundary variation} term $v(\mathbf{p})$ is defined as the variances the surface normals $\mathbf{n}_1, \hdots, \mathbf{n}_n$ along $\psi_{\mathbf{p}} \cap \delta \Omega$ as 
\begin{equation}
v(\mathbf{p})=\frac{1}{3n}\sum_{i=1}^{n}[\mathbf{n}_i-\bar{\mathbf{n}}_i]^T[\mathbf{n}_i-\bar{\mathbf{n}}_i],
\end{equation}
where $\bar{\mathbf{n}}_i$ is the mean vector of $\mathbf{n}_1, \hdots, \mathbf{n}_n$. Large $v(\mathbf{p})$ is an indication of a possible ridge/valley, but it is not sufficient to conclude the presence of such a structure. A true ridge/valley would exhibit a similar profile of normal vectors as one moves away from the boundary $\delta \Omega$ and into $\Omega$. 

To capture this idea, we cluster the surface normals $\mathbf{n}_1, \hdots, \mathbf{n}_n$ of points in $\psi_{\mathbf{p}} \cap \delta \Omega$ following the mean shift clustering algorithm discuss in Section \ref{sec:smooth_patch} and denote the resulting number of clusters $n_{\delta}$. This roughly corresponds to the number of distinct directions of surface normals along the fill front in $\psi_{\mathbf{p}}$. We apply the same (unsupervised) clustering to all normal vectors in $\psi_{\mathbf{p}}$ and denote the resulting number of clusters $n_{\psi}$, which corresponds to the number of distinct directions of normal vectors in the whole $\psi_{\mathbf{p}}$. If the underlying surface exhibits similar profile as one moves away from the boundary within $\psi_{\mathbf{p}}$, we expect $n_{\delta}$ and $n_{\psi}$ to be approximately the same (see Fig.~\ref{fig:normal_vectors}); otherwise $n_{\psi}$ would be larger than $n_{\delta}$. Therefore, the \emph{continuity} term is defined as the ratio of these two numbers, i.e. $c(\mathbf{p})~=n_{\delta}/n_{\psi}$. Finally, the data term is computed as  
\begin{equation}
 D(\mathbf{p})=v(\mathbf{p})c(\mathbf{p}).
\label{eq:dataterm}
\end{equation}

\subsection{Rigid Template matching}
\label{sec:rigid_matching}
Once all priorities on the fill front have been computed, we select the highest priority cube $\psi_{\widehat{\mathbf{p}}}$ as $\widehat{\mathbf{p}} = \arg\max_{\mathbf{p} \in \delta\Omega}P(\mathbf{p})$. Here, the available points in $\psi_{\widehat{\mathbf{p}}}$ are called a \emph{template}. Then we search the source region for the cube $\psi_{\mathbf{q}}$ ($\psi_{\mathbf{q}}\subset \Phi$) that best matches this template. Prior to the actual matching we first reduce the number of candidate cubes as follows.

First, candidate cubes $\psi_{\mathbf{q}}$ that contain fewer points than $\psi_{\widehat{\mathbf{p}}}$ are eliminated from the matching process. After that, further elimination is carried out based on the surface curvature, similar to~\cite{pauly2002}. For the set of points in cube $\psi$, the $3\times 3$ covariance matrix is determined as in~\cite{pauly2002}, and then its eigenvalues $\lambda_{i}$ ($\lambda_{0}\le \lambda_{1}\le \lambda_{2}$) are calculated. The surface curvature within $\psi$ is quantified by 
\begin{equation}
  \sigma(\psi)=\frac{\lambda_{0}}{\lambda_{0}+\lambda_{1}+\lambda_{2}}.
\label{eq:curvature}
\end{equation}
The deviation of the curvatures between $\psi_{\widehat{\mathbf{p}}}$ and a given candidate cube $\psi_{\mathbf{q}}$ is computed as
 \begin{equation}
 e(\psi_{\mathbf{q}})=[\sigma(\psi_{\widehat{\mathbf{p}}})-\sigma(\psi_{\mathbf{q}})]^{2}.
%\label{eq:curvature}
\end{equation}
Here, there is a very high possibility that $e(\psi_{\mathbf{q}})$ get a low value if the cube $\psi_{\mathbf{q}}$ is the best match cube to the $\psi_{\widehat{\mathbf{p}}}$. Therefore, We keep only the 10\% of candidate cubes with lowest $e(\psi_{\mathbf{q}})$ and generate additional candidates by mirroring these cubes through the $xy$ plane. These are used as matching candidates. 

To find the best match for $\psi_{\widehat{p}}$ among the candidate cubes, we proceed is as follows. First, $\psi_{\widehat{\mathbf{p}}}$ is translated such that point $\widehat{\mathbf{p}}$ coincides with the origin. This translated cube is denoted $\overline{\psi}_{\widehat{\mathbf{p}}}$. Then, $\psi_{\mathbf{q}}$ is translated such that point $\mathbf{q}$ coincides with the origin. This translated $\psi_{\mathbf{q}}$ is denoted $\overline{\psi}_{\mathbf{q}}$.  Next, the best 3D rotation matrix $\mathbf{R}_b$  is determined to align $\overline{\psi}_{\mathbf{q}}$ with $\overline{\psi}_{\widehat{\mathbf{p}}}$, and the rotated cube is denoted $\overline{\psi}_{\mathbf{q}}^{\mathbf{R}_b}$. Specifically, the rotation matrix is found as
\begin{equation}
 \mathbf{R}_b=\arg\min_{\mathbf{R}}d(\overline{\psi}_{\mathbf{q}}^{\mathbf{R}}, \overline{\psi}_{\widehat{\mathbf{p}}}),
\label{eq:best_rotation_matrix}
\end{equation}
where $\mathbf{R}$ is a 3D rotation matrix and $d(\overline{\psi}_{\mathbf{q}}^{\mathbf{R}}, \overline{\psi}_{\widehat{\mathbf{p}}})$ is defined as point to point distance (C2C) \cite{tian2017} from $\overline{\psi}_{\widehat{\mathbf{p}}}$ to $\overline{\psi}_{\mathbf{q}}^{\mathbf{R}}$,
\vspace{-4pt}
\begin{equation}
%\vspace{-5pt}
 d(\overline{\psi}_{\mathbf{q}}^{\mathbf{R}}, \overline{\psi}_{\widehat{\mathbf{p}}})=\frac{1}{N_1}\sum_{\mathbf{x}_i \in \overline{\psi}_{\widehat{\mathbf{p}}}}\lVert \mathbf{x}_i-\mathbf{x}_i^{\mathcal{C}} \lVert_2,
\label{eq:C2C}
\vspace{-4pt}
\end{equation}
where $\lVert \cdot \lVert_2$ is the Euclidean norm. Here $N_1$ is the number of points in $\overline{\psi}_{\widehat{\mathbf{p}}}$ and  the point $\mathbf{x}_i^{\mathcal{C}}$ is the closest point in $\overline{\psi}_{\mathbf{q}}^{\mathbf{R}}$ from the point $\mathbf{x}_i$. We use the Iterative Closest Point (ICP) algorithm in~\cite{rusinkiewicz2001} to find $\mathbf{R}_b$ from (\ref{eq:best_rotation_matrix}) for each candidate cube $\overline{\psi}_{\mathbf{q}}$. There are two main steps in ICP.        

\text{Step 1:} Let consider the point set in $\overline{\psi}_{\widehat{\mathbf{p}}}$ as $\{\mathbf{x}_{1},\hdots,\mathbf{x}_{N_1}\}$ and the point set in $\overline{\psi}_{\mathbf{q}}$ as $\{\mathbf{y}_{1},\hdots,\mathbf{y}_{N_1}\}$. At the $k$-th iteration, the rotation matrix is denoted as $\mathbf{R}^{k}$ and then the points set in $\overline{\psi}_{\mathbf{q}}^{\mathbf{R}^{k}}$ is $\{\mathbf{R}^{k}\mathbf{y}_{1},\hdots,\mathbf{R}^{k}\mathbf{y}_{N_1}\}$. For each of the points $\mathbf{x}_i\in \overline{\psi}_{\widehat{\mathbf{p}}}$ the closest point $\mathbf{R}^{k}\mathbf{y}_{i}\in\overline{\psi}_{\mathbf{q}}^{\mathbf{R}^{k}}$ is calculated. Then for each $\mathbf{x}_{i}$ and $\mathbf{R}^{k}\mathbf{y}_{i}$ points, if $\vert|\mathbf{x}_i-\mathbf{R}^{k}\mathbf{y}_{i}|\vert_2$ is less than a given threshold, the pair $(\mathbf{x}_i,\mathbf{y}_i)$ is put into a different set. Afterwards, two matrices $\mathbf{X}$, $\mathbf{Y}$ are constructed so that $\mathbf{X}(:,i)~=~\mathbf{x}_i$ and $\mathbf{Y}(:,i)~=~\mathbf{y}_i$. 

\text{Step 2:} Now we compute the rotation matrix $\mathbf{R}^{k+1}$ which minimizes distance between $(\mathbf{x}_i,\mathbf{y}_i)$ points in matrices $\mathbf{X}$ and $\mathbf{Y}$ as follows:
\begin{equation}
\begin{split}
\mathbf{R}^{k+1}=&\quad \min_{\mathbf{R}}\vert|\mathbf{RY}-\mathbf{X}|\vert_{F}^{2}\\
&\quad \text{s.t.} \hspace{10pt} \mathbf{RR}^T=\mathbf{I}, \det({\mathbf{R}})=1,
\end{split}
\label{eq_ICP_mini}
\end{equation}
where $\lVert \cdot \lVert_F$ is the Frobenius norm. Moreover, $\mathbf{RR}^T~=~\mathbf{I}$ and $\det({\mathbf{R}})=1$ are constraints that $\mathbf{R}$ to be a rotational matrix.  A simple singular value decomposition (SVD) based approach has been proposed in \cite{arun1987} to minimize the expressions as in (\ref{eq_ICP_mini}). According to this SVD based method, $\mathbf{R}^{k+1}$ is computed as
\begin{equation}
\mathbf{R}^{k+1}=\mathbf{VU}^T,
\end{equation}
where SVD of $\mathbf{XY}^T=\mathbf{U\Lambda V}^T$ and it is noted that $\mathbf{XY}^T$ is a $3\times 3$ matrix. These two steps are iteratively repeated until convergence.    

After that, the corresponding C2C after alignment, $d(\overline{\psi}_{\mathbf{q}}^{\mathbf{R}_b}, \overline{\psi}_{\widehat{\mathbf{p}}})$, is recorded. Then the rotated cube with the smallest aligned C2C, $\overline{\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$, can be selected for transfer. Specifically, 
\begin{equation}
 \overline{\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}=\arg\min_{\overline{\psi}_{\mathbf{q}}^{\mathbf{R}_b}}d(\overline{\psi}_{\mathbf{q}}^{\mathbf{R}_b}, \overline{\psi}_{\widehat{\mathbf{p}}}).
\label{eq:best_aligned_cube}
\end{equation}
However, the fixed template cube size, as described above, may be inappropriate in several cases. For example, when the surface is relatively flat near $\widehat{\mathbf{p}}$, small cube size may lead to finding an inaccurate match elsewhere in the model where the surface is also relatively flat. For readers familiar with motion estimation in video, this situation is akin to estimating a motion for a block that does not contain sufficiently strong gradient, and may therefore find many fortuitous matches, most of which are wrong. In such a case, the template needs to be increased in order to capture sufficiently discriminative surface structure. There are also other cases where the surface characteristics near $\widehat{\mathbf{p}}$ are so complicated that even the best-matched cube of a given size is poorly matched to the template, i.e. produces large C2C. Transferring the points from that cube into the hole would not make sense, and it seems more reasonable to try matching with a smaller template size.  
 
To account for the cases mentioned above, we extend template matching with adaptive cube size (ACS) selection. Let $\psi^{n}_{\mathbf{q}}$ be a cube of size $n \times n \times n$ voxels, centered at point $\mathbf{q}$, with edges parallel to the $x,y,z$ axes. The smallest cube size we consider is $n=5$. The initial priority is calculated and the highest priority point $\widehat{\mathbf{p}}$ is found with $n=5$. Following the above procedure, we find the best match $\psi^{n}_{\widehat{\mathbf{q}}} \in \Phi$ for $\psi^{n}_{\widehat{\mathbf{p}}}$. Let the rotated and aligned $\psi^{n}_{\widehat{\mathbf{q}}}$ be denoted $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$, and let the C2C between this cube and the template be $d\left(\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}, \psi^{n}_{\widehat{\mathbf{p}}}\right) = \epsilon$. This $\epsilon$ gives us an idea of what kind of matching error we may hope to find for larger cubes. Based on this, we set a matching threshold $T = 1.0001 \cdot \epsilon$. 

After setting $T$, we create a set $\mathcal{C}=\{\psi^{n}_{\mathbf{q}_1}, \psi^{n}_{\mathbf{q}_2}, ..., \psi^{n}_{\mathbf{q}_N}\}$ of all cubes of size $n$ in $\Phi$, such that $d\left(\overline{{\psi^{n}}}_{\mathbf{q}_i}^{\mathbf{R}_b}, \psi^{n}_{\widehat{\mathbf{p}}}\right) \leq T$. This is a set of candidate cubes that match well with the template of size $n$. Then we increase $n$ and eliminate from $\mathcal{C}$ all cubes whose matching error exceeds $T$ with the new size. The process repeats until we are in a position to make a decision about the best-matched cube. Specifically, we keep increasing $n$ until $\mathcal{C}$ either ends up with only one cube (which is then the best match) or becomes empty. In the latter case, we go back to the previous (lower) cube size and select the cube with the lowest matching error as the best match. The procedure is summarized in Algorithm~\ref{alg:ACS}, where $|\mathcal{C}|$ represents the number of elements in $\mathcal{C}$. In our implementation, the cube size $n$ increases in steps of $2$, as indicated in step~\ref{algostep:size_increment} of the algorithm, but other increment schedules are possible.  
              
\begin{algorithm} [!t]
\begin{algorithmic}[1] 
\STATE Find $\widehat{\mathbf{p}}={\arg\max}_{\mathbf{p}\in \delta \Omega^{t}}P(\mathbf{p})$ and set $n=5$ 
\STATE Find the best-matched cube $\psi^{n}_{\widehat{\mathbf{q}}}$ according to (\ref{eq:best_rotation_matrix})-(\ref{eq:best_aligned_cube})
\STATE Let $\epsilon = d\left(\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}, \psi^{n}_{\widehat{\mathbf{p}}}\right)$ and $T = 1.0001 \cdot \epsilon$
\STATE Initialize $\mathcal{C}=\left\{\psi^{n}_{\mathbf{q}_i} \in \Phi : d\left(\overline{{\psi^{n}}}_{\mathbf{q}_i}^{\mathbf{R}_b}, \psi^{n}_{\widehat{\mathbf{p}}}\right) \leq T\right\}$ 
\WHILE{$|\mathcal{C}|>1$} 
	\STATE $n \leftarrow n+2$ \label{algostep:size_increment}
	\FOR{All $\psi^{n}_{\mathbf{q}_i} \in \mathcal{C}$}
		\IF{$d\left(\overline{{\psi^{n}}}_{\mathbf{q}_i}^{\mathbf{R}_b}, \psi^{n}_{\widehat{\mathbf{p}}}\right) > T$}   
			\STATE Remove $\psi^{n}_{\mathbf{q}_i}$ from $\mathcal{C}$  
		\ENDIF
	\ENDFOR
\ENDWHILE
\IF{$|\mathcal{C}|==1$}
	\STATE The cube in $\mathcal{C}$ (of size $n$) is the best match
\ELSE 
	\STATE Best-matched cube of the previous size is the best match
\ENDIF
\caption{Matching with Adaptive Cube Size}
\label{alg:ACS}
\end{algorithmic}
\end{algorithm}

\subsection{Denoising}
After obtaining cube $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$, we apply our proposed denoise method in Section \ref{sec:denoising} to remove the noises associated with the cube. A summary of this denoising procedure is given in Algorithm \ref{alg:denoising_procedure}. In order to find the $\gamma_{opt}$ we estimate the noise variance $\sigma^2$ first in $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ similar to Section \ref{sec:denoising}. Here we assume that the noise variances of $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ and the whole point cloud are approximately same. Then we estimate the $\sigma^2$ in the point cloud by following Section \ref{sec:noise_estimation}. Finally we compute the $\gamma_{opt}$ using the empirical relationship between $\sigma^2$ and $\gamma_{opt}$. We will discuss more details of finding this empirical relationship in Section \ref{sec:exp}       

{\renewcommand\baselinestretch{0.8}\selectfont        
                  \begin{algorithm} [!t]
                  \begin{algorithmic}[1] 
                  %\STATE Determine number of points in initial fill front $\delta \Omega^{0}$
                  \STATE Perform bipartite graph approximation to $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ and obtain red and blue nodes column vectors $\mathbf{q}_r$ and $\mathbf{q}_b$.
                  \STATE set $\mathbf{p}_r~=~\mathbf{q}_r$ and $\mathbf{p}_b~=~\mathbf{q}_b$. 
                  \WHILE{not converge}
                  \STATE Compute surface normals for points in $\mathbf{p}_r$ using (\ref{eq:normal_linear}).
                  \WHILE{not converge}
                  \STATE Update $\mathbf{p}_r$ by solving (\ref{eq:admm}). 
                  \ENDWHILE
                  \STATE Compute surface normals for points in $\mathbf{p}_b$ using (\ref{eq:normal_linear}).
                  \WHILE{not converge}
                  \STATE Update $\mathbf{p}_b$ by solving (\ref{eq:admm}). 
                  \ENDWHILE
                  \ENDWHILE
                  \caption{Complete Denoising Procedure for $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ }
                  \label{alg:denoising_procedure}
                  \end{algorithmic}
                  \end{algorithm}
                  \par}  


\subsection{Point Transfer}
\label{sec:transfer}
Once obtaining the denoise cube $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$, we need to decide which points to transfer to $\psi_{\widehat{\mathbf{p}}}$. In general, point clouds are not necessarily sampled uniformly in 3D, so it is not straightforward to decide which points correspond to the hole region within $\psi_{\widehat{\mathbf{p}}}$. To make this decision, we first translate $\overline{\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ so that its center coincides with $\widehat{\mathbf{p}}$, and we denote the resulting cube ${\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$. Then we match the points of ${\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ with those of $\psi_{\widehat{\mathbf{p}}}$. Let $\mathbf{x}_{\widehat{\mathbf{p}}} \in \psi_{\widehat{\mathbf{p}}}$ be a point in $\psi_{\widehat{\mathbf{p}}}$. Let $\mathbf{x}_{\widehat{\mathbf{q}}}$ be the closest (by Euclidean distance) point to $\mathbf{x}_{\widehat{\mathbf{p}}}$ within ${\psi'}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$,
%\vspace{-15pt}
\begin{equation}
 \mathbf{x}_{\widehat{\mathbf{q}}}=\arg\min_{\mathbf{x} \in {\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}} \|\mathbf{x} - \mathbf{x}_{\widehat{\mathbf{p}}} \|_2.
\label{eq:matching_point}
\vspace{-5pt}
\end{equation} 
Then we say that $\mathbf{x}_{\widehat{\mathbf{q}}}$ has been matched with $\mathbf{x}_{\widehat{\mathbf{p}}}$ and add it to the set of matched points of ${\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$, denoted $M_{\widehat{\mathbf{q}}}$. Finally, all the unmatched points, ${\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b} \setminus M_{\widehat{\mathbf{q}}}$ are transferred to $\psi_{\widehat{\mathbf{p}}}$ and the fill front is updated. In order to do smooth point transferring, the gap between $M_{\widehat{\mathbf{q}}}$ and $\psi_{\widehat{\mathbf{p}}}$ should be minimum as much as possible. Therefore, we perform a \textit{non-rigid transformation} (NRT) to $\overline{\psi}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ to further align $M_{\widehat{\mathbf{q}}}$ with $\psi_{\widehat{\mathbf{p}}}$ before doing the actual point transferring to the hole.         
\subsection{Non-Rigid Transformation for Template Matching}
%Let $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ the best-matched cube found above, after rotation to align it with $\psi^{n}_{\widehat{\mathbf{p}}}$. Let $M_{\widehat{\mathbf{q}}}$ be the set of points in $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ that are matched with points in $\psi^{n}_{\widehat{\mathbf{p}}}$, according to~(\ref{eq:matching_point}). Further improvement in the alignment of $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ and $\psi^{n}_{\widehat{\mathbf{p}}}$ can be achieved by Non-Rigid Transformation (NRT). 
The main challenge in developing a NRT in this case is finding the appropriate transformation for the unmatched points (i.e., those in $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b} \setminus M_{\widehat{\mathbf{q}}}$). To overcome this challenge, we propose the following strategy: the matched points (those in $M_{\widehat{\mathbf{q}}}$) will be transformed to minimize their distance to their matches in $\psi^{n}_{\widehat{\mathbf{p}}}$, while the unmatched points will be transformed in a way that encourages the smoothness of transformation among neighboring points in $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$.

The NRT we will apply to $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ is a collection of affine transformations $\{\mathbf{T}_{i}\}$, where $\mathbf{T}_{i}$ is a $3 \times 3$ matrix applied to $\mathbf{y}_i \in \overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$. 
For the matched points, we define the \emph{distortion} term 
\begin{equation}
D=\sum_{\mathbf{y}_i \in M_{\widehat{\mathbf{q}}}} \lVert \mathbf{T}_{i}\mathbf{y}_{i}-\mathbf{x}_{i} \lVert_2^{2},
\label{eq:dist_term}
\end{equation}
where $\mathbf{x}_{i} \in \psi^{n}_{\widehat{\mathbf{p}}}$ is the point in $\psi^{n}_{\widehat{\mathbf{p}}}$ matched with $\mathbf{y}_{i}$ according to~(\ref{eq:matching_point}). In order to take unmatched points into account, we construct an undirected $k$-nearest neighbor graph of unity weight with points in $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ as nodes. Let $\mathcal{E}$ be the set of edges in this graph. Then we define the \emph{smoothness} term 
%\vspace{-7pt}
\begin{equation}
%\vspace{-7pt}
 S=\sum_{(i,j) \in \mathcal{E}}\lVert \mathbf{T}_{i}-\mathbf{T}_{j} \lVert_F^2,
\label{eq:stiff_term}
\end{equation}
Finally, the total cost is the combination of the distortion term and the smoothness term,
\begin{equation}
J = D + \lambda S,
\label{eq:cost_func}
\end{equation}
where $\lambda$ is the parameter that allows a trade-off between $D$ and $S$ in the cost function. In our experiments, we set $\lambda=1$. 

The total cost $J$ in~(\ref{eq:cost_func}) is minimized using the optimization framework presented in~\cite{amberg2007}. First, the distortion term in (\ref{eq:dist_term}) is rewritten as
\begin{equation}
D=\sum_{i=1}^{N_2}w_i \lVert \mathbf{T}_{i}\mathbf{v}_i-\mathbf{u}_{i} \lVert_2^{2},
\label{eq:dist_term_general}
\end{equation}
where $\mathbf{v}_{i}\in\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$. Moreover, if $\mathbf{v}_{i}$ is matched with a point in $\psi^{n}_{\widehat{\mathbf{p}}}$, then the corresponding $\mathbf{u}_{i}$ is its match point in $\psi^{n}_{\widehat{\mathbf{p}}}$ and then $w_{i}~=~1$. If $\mathbf{v}_{i} \in \overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ is a unmatched point, the corresponding $\mathbf{u}_{i}$ is its closest point in $\psi^{n}_{\widehat{\mathbf{p}}}$ and then $w_{i}~=~0$. Based on these notations, the distortion term in (\ref{eq:dist_term_general}) can be given using matrix expressions as follows:
\begin{equation}
D=\vert|\mathbf{W}(\mathbf{VT}-\mathbf{U})|\vert_{F}^{2},
\label{eq:distortion_matrix}
\end{equation}
where, $\mathbf{W}~=~\text{diag}(w_1,\hdots,w_{N_{2}})$, $\mathbf{T}~=~[\mathbf{T}_{1}\hdots \mathbf{T}_{N_2}]^{T}$, $\mathbf{V}~=~\text{diag}\left(\mathbf{v}_1^T, \hdots,\mathbf{v}_{N_2}^T\right)$, and $\mathbf{U}~=~[\mathbf{u}_{1}\hdots \mathbf{u}_{N_2}]^{T}$. 

To express the smoothness term in (\ref{eq:stiff_term}) in matrix form, a new matrix $\mathbf{M}\in \mathbb{R}$ is defined. For each edge $(i,j)$, the corresponding row in $\mathbf{M}$ has all zeros except entries $i$ and $j$ have $1$ and $-1$ respectively. With $3\times 3$ identity matrix $\mathbf{I}_3$, the smoothness term in (\ref{eq:stiff_term}) can be written as 
\begin{equation}
S=\vert|(\mathbf{M}\otimes\mathbf{I}_3)\mathbf{T}|\vert_F^2,
\label{eq:smooth_matrix}
\end{equation}
where $\otimes$ denotes the Kronecker product.

Using the matrix expressions in (\ref{eq:distortion_matrix}) and ($\ref{eq:smooth_matrix}$), the total cost $J$ can be written as a quadratic function
\begin{equation}
J=\norm{
\underbrace{\begin{bmatrix}
    \lambda \mathbf{M}\otimes \mathbf{I}_{3} \\
    \mathbf{WV}
\end{bmatrix}}_{\mathbf{A}}
 \mathbf{T}
-
 \underbrace{\begin{bmatrix}
    \mathbf{0}\\
    \mathbf{WU} 
\end{bmatrix}}_{\mathbf{B}}
}^{2}_{F}=\norm{\mathbf{AT}-\mathbf{B}}^{2}_{F}.
\end{equation} 
Therefore we minimize $J$ directly and exactly by setting its derivative (with respect to $\mathbf{T}$) to zero. Then $J$ become minimum at
\begin{equation}
\mathbf{T}=\left(\mathbf{A}^T\mathbf{A}\right)^{-1}\mathbf{A}^T\mathbf{B}.
\end{equation}
The $\mathbf{A}$ is a $(3|\mathcal{E}|+N_2)\times 3N_2$ matrix. For any connected graph $|\mathcal{E}|\geq N_2$. Therefore $\mathbf{A}$ should be rank of $3N_2$, i.e., full rank, so that $\mathbf{A}^T\mathbf{A}$ is invertible. In our case $\mathbf{A}$ is a full rank matrix and the proof is given in Appendix \ref{appn:rank proof} similar to the one given in~\cite{amberg2007}.  
 
After optimal $\mathbf{T}_{i}$'s are found, they are applied to all points in $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$. Then the unmatched points of the transformed $\overline{{\psi^{n}}}_{\widehat{\mathbf{q}}}^{\mathbf{R}_b}$ are found and transferred to $\psi_{\widehat{\mathbf{p}}}$. This completes one iteration of the filling procedure; after this, the fill front $\delta \Omega$ is updated and the process repeated until the hole is filled. The filling stops at
the iteration in which the template covers the entire fill front. This procedure is summarized in Algorithm \ref{alg:fill_procedure} where $\delta \Omega^{t}$ denotes the fill front at iteration $t$. 

{\renewcommand\baselinestretch{0.8}\selectfont        
                  \begin{algorithm} [!t]
                  \begin{algorithmic}[1] 
                  %\STATE Determine number of points in initial fill front $\delta \Omega^{0}$
                  \STATE Set iteration index $t=0$
                  \WHILE{Number of fill front points in the template $<$ number of points in the fill front}
                  \STATE Find $\widehat{p}$.
                  \STATE Obtain the best matching cube to the template.
                  \STATE Denoise the best matching cube.
                  \STATE Apply NRT.  
                  \STATE Match the points according to~(\ref{eq:matching_point}), and transfer unmatched points.
                  \STATE Set $t=t+1$
                  \STATE Update the fill front $\delta \Omega^{t}$.
                  \ENDWHILE
                  \caption{ Complete Geometry Filling Procedure}
                  \label{alg:fill_procedure}
                  \end{algorithmic}
                  \end{algorithm}
                  \par}  
